DFBench: Benchmarking Deepfake Image Detection Capability of Large Multimodal Models

With the rapid advancement of generative models, the realism of AI-generated images has significantly improved, posing critical challenges for verifying digital content authenticity. Current deepfake detection methods often depend on datasets with limited generation models and content diversity that fail to keep pace with the evolving complexity and increasing realism of the AI-generated content. Large multimodal models (LMMs), widely adopted in various vision tasks, have demonstrated strong zero-shot capabilities, yet their potential in deepfake detection remains largely unexplored. To bridge this gap, we present \textbf{DFBench}, a large-scale DeepFake Benchmark featuring (i) broad diversity, including 540,000 images across real, AI-edited, and AI-generated content, (ii) latest model, the fake images are generated by 12 state-of-the-art generation models, and (iii) bidirectional benchmarking and evaluating for both the detection accuracy of deepfake detectors and the evasion capability of generative models. Based on DFBench, we propose \textbf{MoA-DF}, Mixture of Agents for DeepFake detection, leveraging a combined probability strategy from multiple LMMs. MoA-DF achieves state-of-the-art performance, further proving the effectiveness of leveraging LMMs for deepfake detection. Database and codes are publicly available at https://github.com/IntMeGroup/DFBench.

==> figures/distortion.tex <==
\begin{figure*}[t]
    \centering
    \begin{minipage}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/distortion_categories.png}
        \raisebox{6mm}{(a)}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/distortion_heatmap.png}
        \raisebox{6mm}{(b)}
    \end{minipage}
    \vspace{-8mm}
    \caption{(a) Distribution of distortion categories; (b) Heatmap showing the frequency of different distortion types detected across 10 generation models.}
    \vspace{-4mm}
    \label{distortion}
\end{figure*}


==> figures/saliency_example.tex <==
\begin{figure*}
    \centering
    % \vspace{-5mm}
    \includegraphics[width=0.9\textwidth]{figures/saliency_exp_2.png}
    \vspace{-4mm}
    \caption{The predicted saliency maps of LMME3DHF on sample images from Gen3DHF dataset.} 
     \vspace{-1mm}
    \label{saliency_example}
\end{figure*}

==> figures/saliency_exp.tex <==
\begin{figure*}
    \centering
    \vspace{-3mm}
    \includegraphics[width=0.98\textwidth]{figures/saliency_exp_1.png}
    \vspace{-5mm}
    \caption{Qualitative comparisons for different models on our Gen3DHF.} 
     \vspace{-1mm}
    \label{saliency_exp}
\end{figure*}

==> figures/saliency_preprocess.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/saliency_preprocess.png}
     \vspace{-4mm}
    \makebox[\linewidth]{\hspace{0.3cm}(a) \hspace{4cm} (b)}
    \caption{(a) Images with human-annotated distortion points; (b) Generated distortion-aware aliency maps.} 
     \vspace{-4mm}
    \label{saliency_preprocess}
\end{figure}

==> tables/ablation.tex <==
\begin{table*}[h]
% \vspace{-3mm}
  \caption{Ablation study of the proposed LMME3DHF on score prediction and visual question answering performance.}
  \vspace{-3mm}
  \renewcommand\arraystretch{0.95}
  \resizebox{0.85\textwidth}{!}{
  \begin{tabular}{cccc|ccc|ccc|c}
    \toprule
    & \multicolumn{3}{c}{Training Strategy} & \multicolumn{3}{c}{Quality} 
    & \multicolumn{3}{c}{Authenticity} & \multicolumn{1}{c}{Accuracy}
    \\
    \cmidrule(r){2-4} \cmidrule(r){5-7} \cmidrule(r){8-10} \cmidrule(r){11-11}
    \multicolumn{1}{c}{No.} & LoRA$_{r=8}$ (vision) & LoRA$_{r=8}$ (LLM) & Quality Regression
    & SRCC & PLCC & KRCC & SRCC & PLCC & KRCC & (\%)
    \\
    \hline
    \multicolumn{1}{c}{(1)} & \ding{52} & & 
    & 0.0324 & 0.0277 & 0.0251 & 0.0316 & 0.0325 & 0.0258 & 30.86
    \\
    \multicolumn{1}{c}{(2)} & & \ding{52} & 
    & 0.7000 & 0.7573 & 0.5807 & 0.7137 & 0.7627 & 0.5923 & 44.83
    \\
    \multicolumn{1}{c}{(3)} & & & \ding{52}
    & 0.8589 & 0.9345 & 0.6715 & 0.8841 & 0.9469 & 0.7111 & 30.73
    \\
    \multicolumn{1}{c}{(4)} & \ding{52} & \ding{52} & 
    & 0.6976 & 0.7517 & 0.5775 & 0.6917 & 0.7431 & 0.5736 & 41.57
    \\
    \rowcolor{gray!20} \multicolumn{1}{c}{(5)} & & \ding{52} & \ding{52}
    & 0.9028 & 0.9424 & 0.7406 & 0.9234 & 0.9571 & 0.7741 & 54.24
    \\
    \multicolumn{1}{c}{(6)} & \ding{52} & \ding{52} & \ding{52}
    & 0.9052 & 0.9420 & 0.7470 & 0.9226 & 0.9561 & 0.7731 & 53.12
    \\
    \bottomrule
  \end{tabular}
  \label{ablation}}
  % \vspace{-2mm}
  \centering
\end{table*}

==> tables/benchmark.tex <==
\begin{table}[t]
\vspace{-3mm}
\caption{Performance comparisons of the state-of-the-art quality evaluation methods on the Gen3DHF from perspectives of Quality and Authenticity. $\spadesuit$ Handcrafted IQA models, $\diamondsuit$ Deep learning-based IQA models, $\clubsuit$ Deep learning-based VQA models,  $\heartsuit$ LMM-based models. The best results are marked in \textcolor{red}{RED} and the second-best in \textcolor{blue}{BLUE}.
}
\centering
\vspace{-3mm}
\resizebox{0.47\textwidth}{!}{
  \begin{tabular}{l||ccc|ccc}
    \toprule

    \multicolumn{1}{l}{\bf Dimension} &
    \multicolumn{3}{c}{\textbf{Quality}} &
    \multicolumn{3}{c}{\textbf{Authenticity}} 
    \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7}
    \textbf{Methods / Metrics}  
    & \textbf{SRCC}  & \textbf{PLCC}  & \textbf{KRCC}
    & \textbf{SRCC}  & \textbf{PLCC}  & \textbf{KRCC}

\\
\hline
$\spadesuit$ \textbf{BMPRI} \cite{min2018blind}
 & 0.2344 & 0.2728 & 0.1591 
 & 0.2428 & 0.2892 & 0.1662

\\
$\spadesuit$ \textbf{BPRI} \cite{min2017blind} 
& 0.3069  & 0.3530 & 0.2100 
& 0.3050  & 0.3596 & 0.2093 

\\
$\spadesuit$ \textbf{BPRI-PSS} \cite{min2017blind} 
 & 0.2714 & 0.2998 & 0.1857 
 & 0.2711 & 0.3089 & 0.1848 

\\
$\spadesuit$ \textbf{BPRI-LSSs}  \cite{min2017blind}
 & 0.2741 & 0.3077 & 0.1864
 & 0.2736 & 0.3164 & 0.1870

\\
 
$\spadesuit$ \textbf{BPRI-LSSn} \cite{min2017blind} 
 & 0.1121 & 0.0999 & 0.0751
 & 0.1174 & 0.1168 & 0.0783

\\
$\spadesuit$ \textbf{BRISQUE} \cite{mittal2012no} 
 & 0.0989 & 0.0929 & 0.0664
 & 0.1035 & 0.1162 & 0.0679

\\
$\spadesuit$ \textbf{HOSA} \cite{xu2016blind}
 & 0.1479 & 0.1793 & 0.0994
 & 0.1511 & 0.1944 & 0.1019

\\
$\spadesuit$ \textbf{NIQE} \cite{mittal2012making}
 & 0.1107 & 0.1807 & 0.0732
 & 0.1336 & 0.2103 & 0.0896

\\
$\spadesuit$ \textbf{QAC} \cite{xue2013learning}
 & 0.1507 & 0.1858 & 0.1012
 & 0.1555 & 0.2102 & 0.1031

\\
\hline
$\diamondsuit$ \textbf{Resnet-18} \cite{he2016deep}
 & 0.7716 & 0.8087 & 0.5773
 & 0.7743 & 0.8173 & 0.5857

\\
$\diamondsuit$ \textbf{Resnet-34} \cite{he2016deep}
 & 0.7699 & 0.8041 & 0.5761
 & 0.7692 & 0.8054 & 0.5720

\\
$\diamondsuit$ \textbf{Resnet-50} \cite{he2016deep}
 & 0.7649 & 0.7886 & 0.5755
 & 0.7431 & 0.7752 & 0.5524

\\
$\diamondsuit$ \textbf{VGG-16} \cite{simonyan2014very}
 & 0.7891 & 0.8339 & 0.5982
 & 0.8064 & 0.8319 & 0.6122

\\
$\diamondsuit$ \textbf{VGG-19} \cite{simonyan2014very}
 & 0.7950 & 0.8379 & 0.6021
 & 0.8212 & 0.8514 & 0.6298

\\
$\diamondsuit$ \textbf{Swin-T} \cite{liu2021swin}
 & 0.8035 & 0.8476 & 0.6133
 & 0.8302 & 0.8638 & 0.6368

\\
$\diamondsuit$ \textbf{Swin-S} \cite{liu2021swin}
 & 0.8132 & 0.8318 & 0.6311
 & \bf\textcolor{blue}{0.8554} & 0.8589 & \bf\textcolor{blue}{0.6611}

\\
$\diamondsuit$ \textbf{Swin-B} \cite{liu2021swin}
 & 0.7512 & 0.8348 & 0.5688
 & 0.7945 & 0.8565 & 0.6131

\\
$\diamondsuit$ \textbf{Swin-L} \cite{liu2021swin}
 & 0.7961 & 0.8627 & 0.6168
 & 0.8235 & 0.8754 & 0.6450

\\
$\diamondsuit$ \textbf{CNNIQA} \cite{kang2014convolutional}
 & 0.6664 & 0.7027 & 0.4787
 & 0.6321 & 0.6724 & 0.4497

\\
$\diamondsuit$ \textbf{StairIQA} \cite{sun2023blind}
 & 0.8098 & 0.8491 & 0.6189
 & 0.8134 & 0.8376 & 0.6303

\\
$\diamondsuit$ \textbf{HyperIQA} \cite{su2020blindly}
& 0.8106 & 0.8473 & 0.6232
& 0.8164 & 0.8577 & 0.6289

\\
\hline
$\clubsuit$ \textbf{MC3-18} \cite{tran2018closer}
 & 0.8076 & 0.8464 & 0.6166
 & 0.8071 & 0.8439 & 0.6111

\\
$\clubsuit$ \textbf{R2P1D-18} \cite{tran2018closer}
 & 0.7865 & 0.8320 & 0.5941
 & 0.8113 & 0.8364 & 0.6137

\\
$\clubsuit$ \textbf{R3D-18} \cite{tran2018closer}
 & 0.7734 & 0.8102 & 0.5788
 & 0.7932 & 0.8255 & 0.5972

\\
$\clubsuit$ \textbf{Swin3D-T} \cite{liu2022video}
 & \bf\textcolor{blue}{0.8333} & \bf\textcolor{blue}{0.8706} & \bf\textcolor{blue}{0.6473}
 & 0.8413 & \bf\textcolor{blue}{0.8737} & 0.6516

\\
$\clubsuit$ \textbf{Swin3D-S} \cite{liu2022video}
 & 0.7978 & 0.8500 & 0.6064
 & 0.8243 & 0.8623 & 0.6342

\\
$\clubsuit$ \textbf{Swin3D-B} \cite{liu2022video}
 & 0.7922 & 0.8419 & 0.6000
 & 0.8321 & 0.8637 & 0.6381

\\
$\clubsuit$ \textbf{Simple-VQA} \cite{sun2022deep}
 & 0.6371 & 0.6753 & 0.4474
 & 0.5930 & 0.6714 & 0.4177

\\
$\clubsuit$ \textbf{Fast-VQA} \cite{wu2022fast}
 & 0.7538 & 0.7965 & 0.5645
 & 0.7451 & 0.7951 & 0.5551
\\
$\clubsuit$ \textbf{DOVER} \cite{wu2023exploring}
 & 0.6564 & 0.6676 & 0.4639
 & 0.6017 & 0.6815 & 0.4301
 
\\
$\clubsuit$ \textbf{TCSVT-BVQA} \cite{li2022blindly}
 & 0.7858 & 0.7985 & 0.5952
 & 0.7713 & 0.7924 & 0.5816
 
\\
$\clubsuit$ \textbf{VSFA} \cite{li2019quality}
 & 0.7501 & 0.8154 & 0.5671
 & 0.7305 & 0.8010 & 0.5483

\\
\hline
$\heartsuit$ \textbf{VideoChat2 (7B)} \cite{li2023videochat} 
 & 0.1959 & 0.2065 & 0.1367
 & 0.0596 & 0.1769 & 0.0427

\\
$\heartsuit$ \textbf{LLaVA-NeXT (8B)} \cite{li2024llava}
 & 0.0702 & 0.1435 & 0.0550
 & 0.0343 & 0.0414 & 0.0280

\\
$\heartsuit$ \textbf{InternVL2.5 (8B)} \cite{chen2024expanding}
 & 0.1226 & 0.0593 & 0.0935
 & 0.2026 & 0.2245 & 0.1585

\\
$\heartsuit$ \textbf{MiniCPM-V2.6 (8B)} \cite{yao2024minicpm}
 & 0.1331 & 0.1137 & 0.0972
 & 0.0989 & 0.1070 & 0.0710

\\
$\heartsuit$ \textbf{Qwen2-VL (7B)} \cite{wang2024qwen2}
 & 0.1329 & 0.1798 & 0.1079
 & 0.0719 & 0.1695 & 0.0558

\\
$\heartsuit$ \textbf{Video-ChatGPT} \cite{maaz2023video}
 & 0.0355 & 0.0528 & 0.0258
 & 0.0011 & 0.0123 & 0.0004

\\
$\heartsuit$ \textbf{Video-LLaVA} \cite{lin2023video}
 & 0.0586 & 0.0783 & 0.0477
 & 0.1199 & 0.1258 & 0.0978

\\
$\heartsuit$ \textbf{Video-LLaMA2} \cite{cheng2024videollama}
 & 0.1976 & 0.2806 & 0.1547
 & 0.2750 & 0.3035 & 0.2211

\\
\hline
\rowcolor{gray!20}\textbf{LMME3DHF (Ours)} 

& \bf\textcolor{red}{0.9000} & \bf\textcolor{red}{0.9415} & \bf\textcolor{red}{0.7363} 

& \bf\textcolor{red}{0.9203} & \bf\textcolor{red}{0.9555} & \bf\textcolor{red}{0.7694} 

\\
\rowcolor{gray!20}\textit{Improvement} & +6.6\% & +7.1\% & +8.9\% & +6.5\% & +8.2\% & +10.8\%
\\
\bottomrule
\end{tabular}}
\label{benchmark}
% \vspace{-5mm}
\end{table}

==> tables/combine.tex <==
\begin{table*}[ht]
    \caption{Comparison of SIDA with other deepfake detection methods. Values outside parentheses are evaluated with open-source models directly on the SID-Set; values in parentheses indicate performance changes after fine-tuning the models using the SID-Set on the validation set. ${\textcolor{red}{Red}}$ indicates improvement, and ${\textcolor{green}{green}}$ indicates a decrease in performance. The best results are in bold.}
    \small
    % \setlength{\tabcolsep}{4pt} 
    %\renewcommand{\arraystretch}{0.9}
    \centering
    \begin{tabular}{ccccccccccccc}
        \Xhline{1pt}
         \multirow{2}{*}{Methods} &\multicolumn{3}{c}{Real} & \multicolumn{3}{c}{Fully AI} & \multicolumn{3}{c}{Partial AI}& \multicolumn{3}{c}{Overall} \\
         \cmidrule(r){2-4}
         \cmidrule(r){5-7}
         \cmidrule(r){8-10}
         \cmidrule(r){11-13}
         & Acc & F1 & AUC &Acc & F1 & AUC &Acc & F1&AUC&Acc & F1&AUC \\
        \midrule
        AntifakePrompt~\cite{DBLP:journals/corr/abs-2310-17419}   
        & 64.8${\textcolor{red}{\scriptstyle(\uparrow24.1)}}$ 
        & 78.6${\textcolor{red}{\scriptstyle(\uparrow10.5)}}$  
        & 93.8${\textcolor{red}{\scriptstyle(\uparrow3.7)}}$ \phantom 
        & 96.8${\textcolor{red}{\scriptstyle(\uparrow1.1)}}$  \phantom
        & 30.8${\textcolor{red}{\scriptstyle(\uparrow60.1)}}$  
        & 47.2${\textcolor{red}{\scriptstyle(\uparrow33.2)}}$  
        & 63.1${\textcolor{red}{\scriptstyle(\uparrow29.1)}}$  
        & 69.3${\textcolor{red}{\scriptstyle(\uparrow23.4)}}$
        \\
        CnnSpott~\cite{DBLP:journals/corr/abs-2104-02984} 
        
        & 79.8${\textcolor{red}{\scriptstyle(\uparrow9.2)}}$ \phantom
        & 88.7${\textcolor{red}{\scriptstyle(\uparrow2.1)}}$ \phantom 
        & 39.5${\textcolor{red}{\scriptstyle(\uparrow51.2)}}$  
        & 56.6${\textcolor{red}{\scriptstyle(\uparrow31.5)}}$ 
        & 6.9${\textcolor{red}{\scriptstyle(\uparrow61.2)}}$  \phantom
        & 12.9${\textcolor{red}{\scriptstyle(\uparrow51.1)}}$  
        & 42.1${\textcolor{red}{\scriptstyle(\uparrow39.3)}}$  
        & 69.6${\textcolor{red}{\scriptstyle(\uparrow20.7)}}$  
        \\
        FreDect~\cite{DBLP:conf/icml/FrankESFKH20} 
        
        & 83.7${\textcolor{green}{\scriptstyle(\downarrow37.7)}}$ 
        
        & 91.1${\textcolor{green}{\scriptstyle(\downarrow43.5)}}$ 
        & 16.8${\textcolor{red}{\scriptstyle(\uparrow44.1)}}$  
        & 28.8${\textcolor{red}{\scriptstyle(\uparrow37.2)}}$  
        & 11.9${\textcolor{red}{\scriptstyle(\uparrow25.2)}}$  
        & 21.3${\textcolor{red}{\scriptstyle(\uparrow31.7)}}$   
        & 37.4${\textcolor{red}{\scriptstyle(\uparrow33.6)}}$   
        & 23.4${\textcolor{red}{\scriptstyle(\uparrow47.2)}}$   
        \\
       Fusing~\cite{DBLP:conf/icip/JuJKXNL22} 
       
       & 85.1${\textcolor{red}{\scriptstyle(\uparrow4.1)}}$ \phantom 
       & \textbf{92.0${\textcolor{red}{\scriptstyle(\uparrow0.7)}}$ } \phantom
       & 34.0${\textcolor{red}{\scriptstyle(\uparrow54.1)}}$  
       & 50.7${\textcolor{red}{\scriptstyle(\uparrow38.4)}}$  
       & 2.7${\textcolor{red}{\scriptstyle(\uparrow24.3)}}$  
       & 5.3${\textcolor{red}{\scriptstyle(\uparrow26.1)}}$  
       & 40.1${\textcolor{red}{\scriptstyle(\uparrow33.1)}}$  
       & 29.1${\textcolor{red}{\scriptstyle(\uparrow40.3)}}$ 
       \\
        Gram-Net~\cite{DBLP:conf/cvpr/LiuQT20} 
       
        & 70.1${\textcolor{red}{\scriptstyle(\uparrow19.1)}}$ 
        & 82.4${\textcolor{red}{\scriptstyle(\uparrow9.3)}}$ \phantom 
        & 93.5${\textcolor{red}{\scriptstyle(\uparrow4.4)}}$ 
        \phantom
        & 96.6${\textcolor{red}{\scriptstyle(\uparrow2.0)}}$  
        \phantom
        & 0.8${\textcolor{red}{\scriptstyle(\uparrow89.1)}}$ \phantom 
        & 1.6${\textcolor{red}{\scriptstyle(\uparrow85.3)}}$ \phantom 
        & 55.0${\textcolor{red}{\scriptstyle(\uparrow37.1)}}$  
        & 58.0${\textcolor{red}{\scriptstyle(\uparrow35.1)}}$ 
        \\
        UnivFD~\cite{DBLP:conf/cvpr/OjhaLL23} 
       
        & 68.0${\textcolor{red}{\scriptstyle(\uparrow0.3)}}$ \phantom
        & 67.4${\textcolor{red}{\scriptstyle(\uparrow1.1)}}$ \phantom
        & 62.1${\textcolor{red}{\scriptstyle(\uparrow24.3)}}$ 
        & 87.5${\textcolor{red}{\scriptstyle(\uparrow10.5)}}$
        & 64.0${\textcolor{red}{\scriptstyle(\uparrow28.5)}}$ 
        & 85.3${\textcolor{red}{\scriptstyle(\uparrow4.7)}}$ \phantom
        & 64.0${\textcolor{red}{\scriptstyle(\uparrow21.7)}}$ 
        & 85.3${\textcolor{red}{\scriptstyle(\uparrow4.5)}}$
        \phantom{0} 
        \\
        LGrad~\cite{DBLP:conf/cvpr/Tan0WGW23} 
        
        & 64.8${\textcolor{green}{\scriptstyle(\downarrow2.8)}}$ \phantom 
        & 78.6${\textcolor{green}{\scriptstyle(\downarrow2.5)}}$ \phantom
        & 83.5${\textcolor{green}{\scriptstyle(\downarrow25.5)}}$
        & 91.0${\textcolor{green}{\scriptstyle(\downarrow23.7)}}$
        & \textbf{6.8${\textcolor{red}{\scriptstyle(\uparrow\textbf{92.3})}}$} 
        & \textbf{12.7${\textcolor{red}{\scriptstyle(\uparrow\textbf{86.1})}}$}
        & 51.8${\textcolor{red}{\scriptstyle(\uparrow20.2)}}$
        & 55.5${\textcolor{red}{\scriptstyle(\uparrow23.9)}}$
        \\
        LNP~\cite{DBLP:journals/corr/abs-2311-00962} 
        
        & 71.2${\textcolor{green}{\scriptstyle(\downarrow56.8)}}$
        & 83.2${\textcolor{green}{\scriptstyle(\downarrow60.2)}}$ 
        & 91.8${\textcolor{green}{\scriptstyle(\downarrow55.6)}}$ 
        & 95.7${\textcolor{green}{\scriptstyle(\downarrow60.1)}}$ 
        & 2.9${\textcolor{red}{\scriptstyle(\uparrow90.4)}}$ \phantom
        & 5.7${\textcolor{red}{\scriptstyle(\uparrow88.9)}}$ \phantom
        & 55.2${\textcolor{green}{\scriptstyle(\downarrow7.6)}}$
        \phantom
        & 58.2${\textcolor{red}{\scriptstyle(\uparrow4.1)}}$ 
        \phantom{0} 
        \\
        \hline
        SIDA-7B 
        
        & 89.1
        &91.0
        & \textbf{98.7} 
        & 98.6
        & 91.2
        & 91.0 
        & 93.5 
        & \textbf{93.5}
        \\
        SIDA-13B 
       
        & \textbf{89.6}
        & 91.1
        & 98.5 
        & \textbf{98.7}
        & 92.9
        & 91.2 
        & \textbf{93.6}
        & \textbf{93.5}
        \\
        \Xhline{1pt}
        
    \end{tabular}
    \label{tabel:detection}
\end{table*}

==> tables/partial2.tex <==
\begin{table*}
\setlength{\belowcaptionskip}{-0.01cm}
\centering
\belowrulesep=0pt
\aboverulesep=0pt
\renewcommand\arraystretch{1.1}
% \vspace{-6mm}
\caption{{\bf Performance benchmark on AIGVE-60K.} {\it Overall-Averaged} indicates that we average the MOS of the two dimensions as the overall video quality score. $\spadesuit$Conventional handcrafted metrics, $\diamondsuit$VBench metrics, $\clubsuit$deep learning-based VQA models, $\heartsuit$vision-language pre-training models, $\bigstar$open-source LMM-based models, and $\triangle$close-source LMM-based models. $\blacklozenge$*Refers to fine-tuned models. The best results are marked in {\red{RED}} and the second-best in {\blue{BLUE}}. 
% All experiments for AQA and VQA methods are retrained on each dimension under 10 random train-test splits at a ratio of 8:2.
}\vspace{-3mm}
   \resizebox{\linewidth}{!}{\begin{tabular}{l|cc:cc|cc:cc|cc:cc|cc:cc|cc:cc}
    \toprule[1pt]
     %\multicolumn{2}{c}{\bf Training/Testing}&\multicolumn{8}{c}{{\bf GAIA} (9180)}&-\\
     %\midrule
   {\bf Dimension}  & \multicolumn{4}{c|}{\textbf{Style Change}}&\multicolumn{4}{c|}{\textbf{Object Enhancement}}&\multicolumn{4}{c|}{ \textbf{Object Operation}}&\multicolumn{4}{c}{\textbf{Semantic Change}}&\multicolumn{4}{c}{\textbf{Overall}}\\
   \cdashline{2-15}
   \textit{mix with} & \multicolumn{2}{c:}{\textit{Fully AI}} & \multicolumn{2}{c|}{\textit{Real}}& \multicolumn{2}{c:}{\textit{Fully AI}} & \multicolumn{2}{c|}{\textit{Real}}& \multicolumn{2}{c:}{\textit{Fully AI}} & \multicolumn{2}{c|}{\textit{Real}}&\multicolumn{2}{c:}{\textit{Fully AI}} & \multicolumn{2}{c}{\textit{Real}}&\multicolumn{2}{c:}{\textit{Fully AI}} & \multicolumn{2}{c}{\textit{Real}}\\
   \cdashline{2-15}
{\bf Methods / Metrics}&Acc(\%)$\uparrow$&F1$\uparrow$&Acc(\%)$\uparrow$&F1$\uparrow$&Acc(\%)$\uparrow$&F1$\uparrow$&Acc(\%)$\uparrow$&F1$\uparrow$&Acc(\%)$\uparrow$&F1$\uparrow$&Acc(\%)$\uparrow$&F1$\uparrow$&Acc(\%)$\uparrow$&F1$\uparrow$&Acc(\%)$\uparrow$&F1$\uparrow$&Acc(\%)$\uparrow$&F1$\uparrow$&Acc(\%)$\uparrow$&F1$\uparrow$\\
    \midrule
   %  $\spadesuit$BMPRI \cite{quality:BMPRI} &0.5741&0.4976&0.7878&0.7312& 0.3618 &0.3214 &0.7321 &0.6582&0.5106 &0.4452 &0.7709&0.7112 &64.00 &0.7023\\
   %  $\spadesuit$BPRI  \cite{min2017blind}&0.3558 &0.3403 &0.6356 &0.7122 &0.2018& 0.2012 &0.5324 & 0.6256&0.3044&0.2945&0.5800&0.6863&63.56&0.4701\\
   %  $\spadesuit$BRISQUE \cite{mittal2012no} &0.5843&0.4881&0.8131 &0.7196 &0.3806 &0.3325 & 0.7615 & 0.6598&0.5239&0.4459&0.8011&0.7048&64.67&0.7366\\
   % $\spadesuit$HOSA \cite{xu2016blind} &0.6474&0.5642&0.8456&0.7397 &0.4153 & 0.3682 & 0.7780 & 0.6735&0.5773&0.5068&0.8269&0.7226&64.34&0.7571\\
   % $\spadesuit$NIQE \cite{mittal2012making}&0.6536&0.3517&0.8412&0.7500& 0.4345 &0.2544 & 0.7838 & 0.7037 &0.5917&0.3294&0.8251&0.7412&62.21&0.7602\\
   % $\spadesuit$QAC \cite{xue2013learning}&0.5958&0.5717&0.8100&0.7447& 0.3948 & 0.3430 & 0.7717 & 0.6557&0.5421&0.4974&0.8029&0.7182&64.40&0.7495\\
   %  \hdashline
   %  $\diamondsuit$V-Aesthetic Quality~\cite{huang2024vbench}&0.5031 &0.5315 &0.7740 &0.8309 &0.4033 &0.4358 &0.7273 &0.7986 &0.4877 &0.5254 &0.7526& 0.8291&64.54&0.7046\\
   %   $\diamondsuit$V-Imaging Quality~\cite{huang2024vbench}&0.2810 &0.3093 &0.5426 &0.4766 &0.1952 &0.2244 &0.4986 &0.5101 &0.2531 &0.2900 &0.5186 &0.4970&60.60&0.4389\\
   %  $\diamondsuit$V-Overall Consistency~\cite{huang2024vbench}&0.1559 &0.1939 &0.1742 &0.3319 & 0.3076 &0.3685 &0.3201 &0.5419 &0.2510 &0.3046 &0.2338 &0.4233 &61.96&0.3353\\
   %  $\diamondsuit$V-Subject Consistency~\cite{huang2024vbench}& 0.3443 & 0.3968 &0.4839 &0.6065 &0.1647 &0.2425 &0.4416 &0.5744 &0.2739 &0.3476 &0.4679 &0.6016&62.52&0.4545\\
   %   % $\diamondsuit$V-Background Consistency~\cite{huang2024vbench}& 0.3443 & 0.3864 &0.4772 &0.6219 &0.1916 &0.2375 &0.4429 &0.5635 &0.2906 &0.3392 &0.4590 &0.6064&62.37\\
   % $\diamondsuit$V-Temporal Flickering~\cite{huang2024vbench}& 0.4076 &0.4491 &0.6396 &0.6437 &0.1958 &0.2432 &0.5778 &0.5339 &0.3272 &0.3765 &0.6018 &0.6072&63.69&0.5764\\
   %  % $\diamondsuit$Temporal Style~\cite{huang2024vbench}& 0.1559 &0.1939 &0.1742 &0.3319 &0.3076 &0.3685 &0.3201 &0.5419 &0.2510 &0.3046 &0.2338 &0.4233&-\\
   % %  $\clubsuit$Action-Score \cite{liu2023evalcrafter}&&0.2023&0.1823&0.2867&0.2623&0.2689&0.2432&0.2600&0.2377 &-\\
   % % $\clubsuit$Flow-Score \cite{liu2023evalcrafter}& &0.1471&0.1541&0.0816&0.1273&0.1041&0.1309&0.1166&0.1430&-\\
   %     \hdashline
   %  % $\clubsuit$TLVQM \cite{korhonen2019two}&&-\\
   %  % $\clubsuit$VIDEVAL \cite{tu2021ugc}&&-\\
   %  $\clubsuit$VSFA \cite{VSFA}&0.3750 &0.3898 & 0.6227 & 0.5987 &0.2438 &0.2645 &0.5858 &0.5777 &0.3320 &0.3556 &0.6102 &0.5983&57.09&0.5204\\
   %  $\clubsuit$BVQA \cite{li2022blindly}&0.3089 & 0.3512 &0.5030 &0.6506 & 0.2379 & 0.2675 &0.4674 &0.6009 &0.3023 &0.3361 &0.4897 &0.6390&58.47&0.4781\\
   %  $\clubsuit$SimpleVQA \cite{sun2022deep}&0.5631 & 0.5670 & 0.8038 & 0.7873 &0.3474 &0.3487 &0.7273 &0.7327 &0.4884 &0.4979 &0.7620 &0.7756&60.78&0.6894\\
   %  $\clubsuit$FAST-VQA \cite{wu2022fast}&0.6391 & 0.6394 & 0.8945 & 0.9063 & 0.3919 &0.4162 &0.8376 &0.8492 &0.5563 & 0.5738 &0.8683 &0.8952&66.27&0.8122\\ 
   %  $\clubsuit$DOVER \cite{wu2023dover}& 0.6414 & 0.6552 & 0.8874 & 0.9244 &0.3759 &0.3936 &0.8038 &0
   %  .8448 & 0.5480 &0.5702 &0.8496 &0.9043&62.61&0.7662\\
   %   \hdashline
   %   $\heartsuit$CLIPScore~\cite{hessel2021clipscore} &0.0947 &0.1348 &0.0300 &0.1732 &0.2290 & 0.2818 & 0.1408 & 0.3835 &0.1738 &0.2256 &0.0848 &0.2625&58.27&0.1695\\
   %   $\heartsuit$BLIPScore~\cite{li2022blip}&0.1884 &0.2341 &0.2111 &0.3436 &0.3163 &0.3813 & 0.3451 & 0.5354&0.2735 &0.3335 &0.2814 &0.4277&63.93&0.3775\\
   %   $\heartsuit$AestheticScore~\cite{schuhmann2022laion}&0.5524&0.5613 &0.7566 &0.8053 &0.3931 & 0.4149 & 0.7001 & 0.7634 &0.5107 &0.5304 &0.7206 &0.7991&64.87&0.6734\\
   %   % $\heartsuit${\it - - same as the above - -} &&0.3179&0.3101&0.3551&0.3511&0.3504&0.3380&0.3531&0.3458 &-\\
   %   $\heartsuit$ImageReward~\cite{xu2023imagereward}&0.4180 &0.4472 &0.8016 &0.8097 &0.5076 & 0.5419 & 0.8549 & 0.8790&0.4992&0.5365&0.8331&0.8495&68.33&0.8586\\
   %   $\heartsuit$PickScore~\cite{kirstain2023pick}&0.4026 &0.4193 &0.8198 &0.8344 &0.4135 & 0.4246 & 0.7775 & 0.8497&0.4395&0.4580&0.8033&0.8522&62.29&0.7844\\
   %  $\heartsuit$HPSv2~\cite{wu2023human}&0.5415 &0.5690&0.7504&0.8096& 0.4989 & 0.5325 & 0.7522 & 0.8379&0.5605&0.5980&0.7468&0.8325&67.68&0.7789\\
   %  $\heartsuit$VQAScore~\cite{li2024evaluating}&0.1677&0.1961&0.3437&0.3365& 0.1763 & 0.2049 & 0.3922 & 0.4173&0.1880&0.2176&0.3811&0.3746&52.97&0.3280\\
   %  $\heartsuit$FGA-BLIP2~\cite{han2024evalmuse40kreliablefinegrainedbenchmark}&0.5181&0.5340&0.8954&0.8962& 0.5962 & 0.6081 & 0.9502 & 0.9543 &0.6035&0.6196&0.9297&0.9326&67.06&0.9372\\
   %  \hdashline
   %  $\bigstar$DeepseekVL2 (1B)~\cite{wu2024deepseekvl2mixtureofexpertsvisionlanguagemodels}& 0.0121 & 0.0064 & 0.0607 & 0.0427 & 0.0173 & 0.0252& 0.0785 &0.0288&0.0012&0.0137&0.0389&0.0554 & 39.29&0.0965\\
    $\bigstar$VideoLlava (7B)~\cite{lin2023video} & 0.1809 & 0.1938 & 0.6125 & 0.6817 &0.2005&0.2127 &0.6406 &0.6700&0.2026&0.2267&0.6764&0.7505& 68.46&0.7548\\
    $\bigstar$mPLUG-Owl3 (7B)~\cite{ye2024mplug} &0.3532 & 0.3542 & 0.7962 & 0.7789 &0.5478 &0.5551&0.9310 &0.9273&0.5540&0.5626&0.9008&0.8886& 63.02&0.8897\\ 
   $\bigstar$VideoLlama3 (8B)~\cite{damonlpsg2025videollama3} & 0.3922 & 0.4196 & 0.9073 &0.9144&0.4228&0.4817&0.9075&0.8569 &0.5063&0.5432&0.9576&0.9550& 70.16&0.8244\\
   $\bigstar$Qwen2-VL (7B) \cite{wang2024qwen2}&0.3568 &0.3615 &0.7085 &0.7588 &0.4498 &0.4789 &0.7953 &0.8464 &0.4105 &0.4313 &0.7775 &0.8127 &71.56&0.8681\\
 $\bigstar$Qwen2.5-VL (7B)~\cite{Qwen2.5-VL} &0.5410 & 0.5410 & 0.8652 & 0.8683 &0.5110&0.5223&0.8167&0.8692&0.5578&0.5799&0.8888&0.8949&62.34&0.6655\\
   $\bigstar$Llama3.2-Vision (11B)~\cite{meta2024llama} & 0.0940 & 0.0752 & 0.4483 & 0.5023 &0.0804&0.0530&0.2783&0.1784
    &0.1064&0.0792&0.4061&0.4294& 62.19&0.6033\\
  $\bigstar$CogAgent (18B)~\cite{hong2024cogagentvisuallanguagemodel} & 0.1244 & 0.1242 &0.4834 & 0.5906 &0.1190&0.1129&0.8198&0.8363&0.1481&0.1471&0.6311&0.7133& 65.32&0.7763\\
    $\bigstar$InternVL2.5 (8B)~\cite{chen2024expanding} & 0.2799 & 0.3336 & 0.7882 & 0.7978&0.4856&0.5268&0.9390&0.9483&0.4715&0.5164&0.9057&0.9084& 66.30&0.8051\\
    $\bigstar$InternVL3 (9B)~\cite{wang2024mpo} & 0.2731 &0.3519 &0.8300 &0.7576 & 0.4768 &0.5334 &0.9373 &0.9610 &0.4793 & 0.5307 & 0.9270 &0.9224& 65.82&0.7719\\
   $\bigstar$InternVideo2.5 (8B)~\cite{wang2025internvideo} & 0.1563 & 0.5454 &0.3361 &0.6574 &0.4978&0.5538&0.9560&0.9646 &0.4430&0.5366&0.9079&0.8968& 70.64&0.8435\\
   $\bigstar$LLaVA-NeXT (8B)~\cite{liu2024llavanext} &0.4888 & 0.5002 &0.8785 &0.8956 &0.2847&0.3090&0.8042&0.8510&0.4910&0.5194& 0.8630&0.9116& 70.21&0.9201\\
   $\bigstar$InternVL2.5 (38B)~\cite{chen2024expanding} &0.6227 &0.5766 &0.9052 &0.8814 &0.6470 &0.6417 &0.9586 &0.9646 &0.6627 &0.6497 &0.9471 &0.9330 &75.81 &0.9456\\
   $\bigstar$InternVL3 (38B)~\cite{wang2024mpo}
   &0.4950 &0.5150 &0.8118 &0.8082 & 0.5996 &0.5920 &0.9439 &0.9463 &0.6040 &0.5984 &0.9128 &0.8946 &73.89 &0.9386\\
   $\bigstar$Qwen2-VL (72B) \cite{wang2024qwen2}&0.4628 &0.5333 &0.8388 &0.8263 &0.5598 &0.5720 &0.9271 &0.9444 &0.5948 &0.6237 &0.9382 &0.9239 &73.12 &0.9064\\
   $\bigstar$Qwen2.5-VL (72B)~\cite{Qwen2.5-VL}&0.4245&0.4562&0.7762&0.7602& 0.6272 &0.5884 &0.9364 &0.9522 &0.5891 &0.5794 &0.9239 &0.9083 &73.83 &0.9516\\
   $\bigstar$Llava-one-vision (72B)~\cite{xiong2024llavaovchat} &0.5291 &0.5196 &0.7829 &0.7689 &0.5702 &0.5510 &0.8741 &0.9055 &0.6010 &0.5827 &0.8478 & 0.8497 &73.31 &0.9112\\
   $\bigstar$InternVL2.5 (72B)~\cite{chen2024expanding} & 0.5383 &0.5394 &0.8843 &0.8303 &0.6612 &0.6326 &0.9542 &0.9513& 0.6417 &0.6324 &0.9146 &0.9039 &75.18&0.9423\\
   $\bigstar$InternVL3 (72B)~\cite{wang2024mpo} & 0.5441 &0.4973 &0.8923 &0.8131 & 0.6314 & 0.6055 &0.9444 &0.9529 &0.6405 &0.6047 &0.9212 &0.9014 & 74.59&0.9623\\
    \hdashline
     $\triangle$Gemini1.5-pro \cite{Gemini}& 0.4972 &0.5012 &0.8790 &0.7965 &0.6095 &0.5874 &0.9430 &0.9491 & 0.5957 &0.5985 &0.9346 &0.9196& 73.38&0.9512\\
     $\triangle$Claude3.5 \cite{Claude3.5}& 0.4267 &0.4711 &0.7602 &0.7343 &0.5827 &0.5809 &0.8919 &0.9238 &0.5532 &0.5822 &0.8598 &0.8481& 73.20&0.9395\\
     $\triangle$Grok2 Vision \cite{Grok2}& 0.5628 &0.5728 &0.8808 &0.8403 &0.6659 &0.6730 &0.9546 &0.9763 &0.6629 &0.6784&0.9399 &0.9368& 76.51&0.9469\\
     $\triangle$ChatGPT-4o \cite{GPT4}& 0.5263 &0.5233 &0.9048 &0.8905 &0.6639 &0.6343 &0.9458 &0.9555&0.6240 &0.6117 &0.9346 &0.9326& 74.84&0.9317\\
     \hdashline
     % $\blacklozenge$Qwen2.5-VL* (7B)~\cite{Qwen2.5-VL} &-\\
    $\blacklozenge$InternVL3* (9B)~\cite{wang2024mpo} & 0.6421 & 0.6575 &0.9061 & 0.9426 &0.5965 &0.6115 & \blue{0.9671} &0.9659 & 0.6571 & 0.6926 & 0.9341 &0.9597 & \blue{78.36}&\blue{0.9754}\\
    $\blacklozenge$Qwen2.5-VL* (7B)~\cite{Qwen2.5-VL} &\blue{0.7868} &0.7996 & 0.9265 &0.9510 & \blue{0.7354} &\blue{0.7493} &0.9634 &0.9677 & 0.7798& 0.8046& \blue{0.9579} & 0.9716 &77.35 &0.9698\\
    $\blacklozenge$InternVideo2.5* (8B)~\cite{wang2025internvideo} & 0.7845 & \blue{0.8102} &\blue{0.9308} & \blue{0.9605} &0.6773 &0.6946 & 0.9608 &\blue{0.9679} & \blue{0.7802} & \blue{0.8094} & 0.9542 &\blue{0.9721} & 73.37 &0.9136\\
     \rowcolor{gray!20} $\blacklozenge$LOVE (Ours) &\red{0.7932} &\red{0.8259}&\red{0.9324}&\red{0.9725}&\red{0.7466} &\red{0.7657} &\red{0.9778} &\red{0.9825} &\red{0.8115}&\red{0.8361}&\red{0.9657}&\red{0.9779} & \red{78.69}&\red{0.9769}\\
% $\bigstar$\textbf{LLaVA-1.5 (7B)}~\cite{wang2025internvideo}
% & 0.3372 & 0.3525 & 0.2577 & 0.3887 
% &-\\
% $\bigstar$\textbf{LLaVA-NeXT (8B)}~\cite{liu2024llavanext}
% & 0.4333 & 0.4164 & 0.3442 & 0.4568 

% &-\\
% $\bigstar$\textbf{mPLUG-Owl3 (7B)}~\cite{ye2024mplug}
% & 0.3918 & 0.3569 & 0.3018 & 0.4744 
% &-\\
% $\bigstar$\textbf{MiniCPM-V2.6 (8B)}~\cite{damonlpsg2025videollama3}
% & 0.3733 & 0.1053 & 0.2839 & 0.5916 
% &-\\
% $\bigstar$\textbf{Qwen2-VL (7B)}~\cite{Qwen2-VL}
% & 0.3760 & 0.3625 & 0.3061 & 0.5899
% &-\\
% % $\clubsuit$\textbf{ MiniCPM-V2.6} \cite{}
% % & 0.3733 & 0.1053 & 0.2839 & 0.5916 & 0.5971 & 0.4597
% % &-\\


% $\bigstar$ \textbf{DeepSeekVL (7B)}~\cite{wu2024deepseekvl2mixtureofexpertsvisionlanguagemodels}
% & 0.2611 & 0.3010 & 0.1988
% & 0.2356 
 
% &-\\
    \bottomrule[1pt]
  \end{tabular}}
  \label{mos}
  % \vspace{-2em}
\end{table*}

==> tables/qa_benchmark.tex <==
\begin{table}
  \caption{Performance comparisons of LMMs on visual question-answering tasks. The best results are marked in \textcolor{red}{RED} and the second-best in \textcolor{blue}{BLUE}.}
  \label{qa_benchamrk}
  \centering
  \vspace{-3mm}
  \begin{tabular}{l|c}
    \toprule
    \textbf{Models} & \textbf{Accuracy (\%)}
    \\
    \midrule
    \textbf{VideoChat2 (7B)} \cite{li2023videochat}  & 16.63
    \\
    \textbf{InternVL2.5 (8B)} \cite{chen2024expanding} & \bf\textcolor{blue}{45.24}
    \\
    \textbf{MiniCPM-V2.6 (8B)} \cite{yao2024minicpm} & 13.83
    \\
    \textbf{Qwen2-VL (7B)} \cite{wang2024qwen2} & 23.18
    \\
    \textbf{Video-ChatGPT} \cite{maaz2023video} & 8.490
    \\
    \bottomrule
    \rowcolor{gray!20}\textbf{LMME3DHF (Ours)} & \bf\textcolor{red}{54.24}
    \\
    \bottomrule
  \end{tabular}
% \vspace{-5mm}
\end{table}

==> tables/real.tex <==
\begin{table*}
\setlength{\belowcaptionskip}{-0.01cm}
\centering
\belowrulesep=0pt
\aboverulesep=0pt
\renewcommand\arraystretch{1.1}
% \vspace{-6mm}
\caption{{\bf Performance benchmark on AIGVE-60K.} {\it Overall-Averaged} indicates that we average the MOS of the two dimensions as the overall video quality score. $\spadesuit$Conventional handcrafted metrics, $\diamondsuit$VBench metrics, $\clubsuit$deep learning-based VQA models, $\heartsuit$vision-language pre-training models, $\bigstar$open-source LMM-based models, and $\triangle$close-source LMM-based models. $\blacklozenge$*Refers to fine-tuned models. The best results are marked in {\red{RED}} and the second-best in {\blue{BLUE}}. 
% All experiments for AQA and VQA methods are retrained on each dimension under 10 random train-test splits at a ratio of 8:2.
}\vspace{-3mm}
   \resizebox{\linewidth}{!}{\begin{tabular}{l|cc:cc|cc:cc|cc:cc|cc:cc|cc:cc}
    \toprule[1pt]
     %\multicolumn{2}{c}{\bf Training/Testing}&\multicolumn{8}{c}{{\bf GAIA} (9180)}&-\\
     %\midrule
   {\bf Dimension}  & \multicolumn{4}{c|}{\textbf{LIVE}}&\multicolumn{4}{c|}{\textbf{CSIQ}}&\multicolumn{4}{c|}{ \textbf{TID2023}}&\multicolumn{4}{c}{\textbf{KADID}}&\multicolumn{4}{c}{\textbf{CLIVE}}\\
   \cdashline{2-15}
   \textit{mix with} & \multicolumn{2}{c:}{\textit{Fully AI}} & \multicolumn{2}{c|}{\textit{Partial AI}}& \multicolumn{2}{c:}{\textit{Fully AI}} & \multicolumn{2}{c|}{\textit{Partial AI}}& \multicolumn{2}{c:}{\textit{Fully AI}} & \multicolumn{2}{c|}{\textit{Partial AI}}&\multicolumn{2}{c:}{\textit{Fully AI}} & \multicolumn{2}{c}{\textit{Partial AI}}&\multicolumn{2}{c:}{\textit{Fully AI}} & \multicolumn{2}{c}{\textit{Partial AI}}\\
   \cdashline{2-15}
{\bf Methods / Metrics}&Acc$\uparrow$&F1$\uparrow$&Acc$\uparrow$&F1$\uparrow$&Acc$\uparrow$&F1$\uparrow$&Acc$\uparrow$&F1$\uparrow$&Acc$\uparrow$&F1$\uparrow$&Acc$\uparrow$&F1$\uparrow$&Acc$\uparrow$&F1$\uparrow$&Acc$\uparrow$&F1$\uparrow$&Acc$\uparrow$&F1$\uparrow$&Acc$\uparrow$&F1$\uparrow$\\
    \midrule
   %  $\spadesuit$BMPRI \cite{quality:BMPRI} &0.5741&0.4976&0.7878&0.7312& 0.3618 &0.3214 &0.7321 &0.6582&0.5106 &0.4452 &0.7709&0.7112 &64.00 &0.7023\\
   %  $\spadesuit$BPRI  \cite{min2017blind}&0.3558 &0.3403 &0.6356 &0.7122 &0.2018& 0.2012 &0.5324 & 0.6256&0.3044&0.2945&0.5800&0.6863&63.56&0.4701\\
   %  $\spadesuit$BRISQUE \cite{mittal2012no} &0.5843&0.4881&0.8131 &0.7196 &0.3806 &0.3325 & 0.7615 & 0.6598&0.5239&0.4459&0.8011&0.7048&64.67&0.7366\\
   % $\spadesuit$HOSA \cite{xu2016blind} &0.6474&0.5642&0.8456&0.7397 &0.4153 & 0.3682 & 0.7780 & 0.6735&0.5773&0.5068&0.8269&0.7226&64.34&0.7571\\
   % $\spadesuit$NIQE \cite{mittal2012making}&0.6536&0.3517&0.8412&0.7500& 0.4345 &0.2544 & 0.7838 & 0.7037 &0.5917&0.3294&0.8251&0.7412&62.21&0.7602\\
   % $\spadesuit$QAC \cite{xue2013learning}&0.5958&0.5717&0.8100&0.7447& 0.3948 & 0.3430 & 0.7717 & 0.6557&0.5421&0.4974&0.8029&0.7182&64.40&0.7495\\
   %  \hdashline
   %  $\diamondsuit$V-Aesthetic Quality~\cite{huang2024vbench}&0.5031 &0.5315 &0.7740 &0.8309 &0.4033 &0.4358 &0.7273 &0.7986 &0.4877 &0.5254 &0.7526& 0.8291&64.54&0.7046\\
   %   $\diamondsuit$V-Imaging Quality~\cite{huang2024vbench}&0.2810 &0.3093 &0.5426 &0.4766 &0.1952 &0.2244 &0.4986 &0.5101 &0.2531 &0.2900 &0.5186 &0.4970&60.60&0.4389\\
   %  $\diamondsuit$V-Overall Consistency~\cite{huang2024vbench}&0.1559 &0.1939 &0.1742 &0.3319 & 0.3076 &0.3685 &0.3201 &0.5419 &0.2510 &0.3046 &0.2338 &0.4233 &61.96&0.3353\\
   %  $\diamondsuit$V-Subject Consistency~\cite{huang2024vbench}& 0.3443 & 0.3968 &0.4839 &0.6065 &0.1647 &0.2425 &0.4416 &0.5744 &0.2739 &0.3476 &0.4679 &0.6016&62.52&0.4545\\
   %   % $\diamondsuit$V-Background Consistency~\cite{huang2024vbench}& 0.3443 & 0.3864 &0.4772 &0.6219 &0.1916 &0.2375 &0.4429 &0.5635 &0.2906 &0.3392 &0.4590 &0.6064&62.37\\
   % $\diamondsuit$V-Temporal Flickering~\cite{huang2024vbench}& 0.4076 &0.4491 &0.6396 &0.6437 &0.1958 &0.2432 &0.5778 &0.5339 &0.3272 &0.3765 &0.6018 &0.6072&63.69&0.5764\\
   %  % $\diamondsuit$Temporal Style~\cite{huang2024vbench}& 0.1559 &0.1939 &0.1742 &0.3319 &0.3076 &0.3685 &0.3201 &0.5419 &0.2510 &0.3046 &0.2338 &0.4233&-\\
   % %  $\clubsuit$Action-Score \cite{liu2023evalcrafter}&&0.2023&0.1823&0.2867&0.2623&0.2689&0.2432&0.2600&0.2377 &-\\
   % % $\clubsuit$Flow-Score \cite{liu2023evalcrafter}& &0.1471&0.1541&0.0816&0.1273&0.1041&0.1309&0.1166&0.1430&-\\
   %     \hdashline
   %  % $\clubsuit$TLVQM \cite{korhonen2019two}&&-\\
   %  % $\clubsuit$VIDEVAL \cite{tu2021ugc}&&-\\
   %  $\clubsuit$VSFA \cite{VSFA}&0.3750 &0.3898 & 0.6227 & 0.5987 &0.2438 &0.2645 &0.5858 &0.5777 &0.3320 &0.3556 &0.6102 &0.5983&57.09&0.5204\\
   %  $\clubsuit$BVQA \cite{li2022blindly}&0.3089 & 0.3512 &0.5030 &0.6506 & 0.2379 & 0.2675 &0.4674 &0.6009 &0.3023 &0.3361 &0.4897 &0.6390&58.47&0.4781\\
   %  $\clubsuit$SimpleVQA \cite{sun2022deep}&0.5631 & 0.5670 & 0.8038 & 0.7873 &0.3474 &0.3487 &0.7273 &0.7327 &0.4884 &0.4979 &0.7620 &0.7756&60.78&0.6894\\
   %  $\clubsuit$FAST-VQA \cite{wu2022fast}&0.6391 & 0.6394 & 0.8945 & 0.9063 & 0.3919 &0.4162 &0.8376 &0.8492 &0.5563 & 0.5738 &0.8683 &0.8952&66.27&0.8122\\ 
   %  $\clubsuit$DOVER \cite{wu2023dover}& 0.6414 & 0.6552 & 0.8874 & 0.9244 &0.3759 &0.3936 &0.8038 &0
   %  .8448 & 0.5480 &0.5702 &0.8496 &0.9043&62.61&0.7662\\
   %   \hdashline
   %   $\heartsuit$CLIPScore~\cite{hessel2021clipscore} &0.0947 &0.1348 &0.0300 &0.1732 &0.2290 & 0.2818 & 0.1408 & 0.3835 &0.1738 &0.2256 &0.0848 &0.2625&58.27&0.1695\\
   %   $\heartsuit$BLIPScore~\cite{li2022blip}&0.1884 &0.2341 &0.2111 &0.3436 &0.3163 &0.3813 & 0.3451 & 0.5354&0.2735 &0.3335 &0.2814 &0.4277&63.93&0.3775\\
   %   $\heartsuit$AestheticScore~\cite{schuhmann2022laion}&0.5524&0.5613 &0.7566 &0.8053 &0.3931 & 0.4149 & 0.7001 & 0.7634 &0.5107 &0.5304 &0.7206 &0.7991&64.87&0.6734\\
   %   % $\heartsuit${\it - - same as the above - -} &&0.3179&0.3101&0.3551&0.3511&0.3504&0.3380&0.3531&0.3458 &-\\
   %   $\heartsuit$ImageReward~\cite{xu2023imagereward}&0.4180 &0.4472 &0.8016 &0.8097 &0.5076 & 0.5419 & 0.8549 & 0.8790&0.4992&0.5365&0.8331&0.8495&68.33&0.8586\\
   %   $\heartsuit$PickScore~\cite{kirstain2023pick}&0.4026 &0.4193 &0.8198 &0.8344 &0.4135 & 0.4246 & 0.7775 & 0.8497&0.4395&0.4580&0.8033&0.8522&62.29&0.7844\\
   %  $\heartsuit$HPSv2~\cite{wu2023human}&0.5415 &0.5690&0.7504&0.8096& 0.4989 & 0.5325 & 0.7522 & 0.8379&0.5605&0.5980&0.7468&0.8325&67.68&0.7789\\
   %  $\heartsuit$VQAScore~\cite{li2024evaluating}&0.1677&0.1961&0.3437&0.3365& 0.1763 & 0.2049 & 0.3922 & 0.4173&0.1880&0.2176&0.3811&0.3746&52.97&0.3280\\
   %  $\heartsuit$FGA-BLIP2~\cite{han2024evalmuse40kreliablefinegrainedbenchmark}&0.5181&0.5340&0.8954&0.8962& 0.5962 & 0.6081 & 0.9502 & 0.9543 &0.6035&0.6196&0.9297&0.9326&67.06&0.9372\\
   %  \hdashline
   %  $\bigstar$DeepseekVL2 (1B)~\cite{wu2024deepseekvl2mixtureofexpertsvisionlanguagemodels}& 0.0121 & 0.0064 & 0.0607 & 0.0427 & 0.0173 & 0.0252& 0.0785 &0.0288&0.0012&0.0137&0.0389&0.0554 & 39.29&0.0965\\
    $\bigstar$VideoLlava (7B)~\cite{lin2023video} & 0.1809 & 0.1938 & 0.6125 & 0.6817 &0.2005&0.2127 &0.6406 &0.6700&0.2026&0.2267&0.6764&0.7505& 68.46&0.7548\\
    $\bigstar$mPLUG-Owl3 (7B)~\cite{ye2024mplug} &0.3532 & 0.3542 & 0.7962 & 0.7789 &0.5478 &0.5551&0.9310 &0.9273&0.5540&0.5626&0.9008&0.8886& 63.02&0.8897\\ 
   $\bigstar$VideoLlama3 (8B)~\cite{damonlpsg2025videollama3} & 0.3922 & 0.4196 & 0.9073 &0.9144&0.4228&0.4817&0.9075&0.8569 &0.5063&0.5432&0.9576&0.9550& 70.16&0.8244\\
   $\bigstar$Qwen2-VL (7B) \cite{wang2024qwen2}&0.3568 &0.3615 &0.7085 &0.7588 &0.4498 &0.4789 &0.7953 &0.8464 &0.4105 &0.4313 &0.7775 &0.8127 &71.56&0.8681\\
 $\bigstar$Qwen2.5-VL (7B)~\cite{Qwen2.5-VL} &0.5410 & 0.5410 & 0.8652 & 0.8683 &0.5110&0.5223&0.8167&0.8692&0.5578&0.5799&0.8888&0.8949&62.34&0.6655\\
   $\bigstar$Llama3.2-Vision (11B)~\cite{meta2024llama} & 0.0940 & 0.0752 & 0.4483 & 0.5023 &0.0804&0.0530&0.2783&0.1784
    &0.1064&0.0792&0.4061&0.4294& 62.19&0.6033\\
  $\bigstar$CogAgent (18B)~\cite{hong2024cogagentvisuallanguagemodel} & 0.1244 & 0.1242 &0.4834 & 0.5906 &0.1190&0.1129&0.8198&0.8363&0.1481&0.1471&0.6311&0.7133& 65.32&0.7763\\
    $\bigstar$InternVL2.5 (8B)~\cite{chen2024expanding} & 0.2799 & 0.3336 & 0.7882 & 0.7978&0.4856&0.5268&0.9390&0.9483&0.4715&0.5164&0.9057&0.9084& 66.30&0.8051\\
    $\bigstar$InternVL3 (9B)~\cite{wang2024mpo} & 0.2731 &0.3519 &0.8300 &0.7576 & 0.4768 &0.5334 &0.9373 &0.9610 &0.4793 & 0.5307 & 0.9270 &0.9224& 65.82&0.7719\\
   $\bigstar$InternVideo2.5 (8B)~\cite{wang2025internvideo} & 0.1563 & 0.5454 &0.3361 &0.6574 &0.4978&0.5538&0.9560&0.9646 &0.4430&0.5366&0.9079&0.8968& 70.64&0.8435\\
   $\bigstar$LLaVA-NeXT (8B)~\cite{liu2024llavanext} &0.4888 & 0.5002 &0.8785 &0.8956 &0.2847&0.3090&0.8042&0.8510&0.4910&0.5194& 0.8630&0.9116& 70.21&0.9201\\
   $\bigstar$InternVL2.5 (38B)~\cite{chen2024expanding} &0.6227 &0.5766 &0.9052 &0.8814 &0.6470 &0.6417 &0.9586 &0.9646 &0.6627 &0.6497 &0.9471 &0.9330 &75.81 &0.9456\\
   $\bigstar$InternVL3 (38B)~\cite{wang2024mpo}
   &0.4950 &0.5150 &0.8118 &0.8082 & 0.5996 &0.5920 &0.9439 &0.9463 &0.6040 &0.5984 &0.9128 &0.8946 &73.89 &0.9386\\
   $\bigstar$Qwen2-VL (72B) \cite{wang2024qwen2}&0.4628 &0.5333 &0.8388 &0.8263 &0.5598 &0.5720 &0.9271 &0.9444 &0.5948 &0.6237 &0.9382 &0.9239 &73.12 &0.9064\\
   $\bigstar$Qwen2.5-VL (72B)~\cite{Qwen2.5-VL}&0.4245&0.4562&0.7762&0.7602& 0.6272 &0.5884 &0.9364 &0.9522 &0.5891 &0.5794 &0.9239 &0.9083 &73.83 &0.9516\\
   $\bigstar$Llava-one-vision (72B)~\cite{xiong2024llavaovchat} &0.5291 &0.5196 &0.7829 &0.7689 &0.5702 &0.5510 &0.8741 &0.9055 &0.6010 &0.5827 &0.8478 & 0.8497 &73.31 &0.9112\\
   $\bigstar$InternVL2.5 (72B)~\cite{chen2024expanding} & 0.5383 &0.5394 &0.8843 &0.8303 &0.6612 &0.6326 &0.9542 &0.9513& 0.6417 &0.6324 &0.9146 &0.9039 &75.18&0.9423\\
   $\bigstar$InternVL3 (72B)~\cite{wang2024mpo} & 0.5441 &0.4973 &0.8923 &0.8131 & 0.6314 & 0.6055 &0.9444 &0.9529 &0.6405 &0.6047 &0.9212 &0.9014 & 74.59&0.9623\\
    \hdashline
     $\triangle$Gemini1.5-pro \cite{Gemini}& 0.4972 &0.5012 &0.8790 &0.7965 &0.6095 &0.5874 &0.9430 &0.9491 & 0.5957 &0.5985 &0.9346 &0.9196& 73.38&0.9512\\
     $\triangle$Claude3.5 \cite{Claude3.5}& 0.4267 &0.4711 &0.7602 &0.7343 &0.5827 &0.5809 &0.8919 &0.9238 &0.5532 &0.5822 &0.8598 &0.8481& 73.20&0.9395\\
     $\triangle$Grok2 Vision \cite{Grok2}& 0.5628 &0.5728 &0.8808 &0.8403 &0.6659 &0.6730 &0.9546 &0.9763 &0.6629 &0.6784&0.9399 &0.9368& 76.51&0.9469\\
     $\triangle$ChatGPT-4o \cite{GPT4}& 0.5263 &0.5233 &0.9048 &0.8905 &0.6639 &0.6343 &0.9458 &0.9555&0.6240 &0.6117 &0.9346 &0.9326& 74.84&0.9317\\
     \hdashline
     % $\blacklozenge$Qwen2.5-VL* (7B)~\cite{Qwen2.5-VL} &-\\
    $\blacklozenge$InternVL3* (9B)~\cite{wang2024mpo} & 0.6421 & 0.6575 &0.9061 & 0.9426 &0.5965 &0.6115 & \blue{0.9671} &0.9659 & 0.6571 & 0.6926 & 0.9341 &0.9597 & \blue{78.36}&\blue{0.9754}\\
    $\blacklozenge$Qwen2.5-VL* (7B)~\cite{Qwen2.5-VL} &\blue{0.7868} &0.7996 & 0.9265 &0.9510 & \blue{0.7354} &\blue{0.7493} &0.9634 &0.9677 & 0.7798& 0.8046& \blue{0.9579} & 0.9716 &77.35 &0.9698\\
    $\blacklozenge$InternVideo2.5* (8B)~\cite{wang2025internvideo} & 0.7845 & \blue{0.8102} &\blue{0.9308} & \blue{0.9605} &0.6773 &0.6946 & 0.9608 &\blue{0.9679} & \blue{0.7802} & \blue{0.8094} & 0.9542 &\blue{0.9721} & 73.37 &0.9136\\
     \rowcolor{gray!20} $\blacklozenge$LOVE (Ours) &\red{0.7932} &\red{0.8259}&\red{0.9324}&\red{0.9725}&\red{0.7466} &\red{0.7657} &\red{0.9778} &\red{0.9825} &\red{0.8115}&\red{0.8361}&\red{0.9657}&\red{0.9779} & \red{78.69}&\red{0.9769}\\
% $\bigstar$\textbf{LLaVA-1.5 (7B)}~\cite{wang2025internvideo}
% & 0.3372 & 0.3525 & 0.2577 & 0.3887 
% &-\\
% $\bigstar$\textbf{LLaVA-NeXT (8B)}~\cite{liu2024llavanext}
% & 0.4333 & 0.4164 & 0.3442 & 0.4568 

% &-\\
% $\bigstar$\textbf{mPLUG-Owl3 (7B)}~\cite{ye2024mplug}
% & 0.3918 & 0.3569 & 0.3018 & 0.4744 
% &-\\
% $\bigstar$\textbf{MiniCPM-V2.6 (8B)}~\cite{damonlpsg2025videollama3}
% & 0.3733 & 0.1053 & 0.2839 & 0.5916 
% &-\\
% $\bigstar$\textbf{Qwen2-VL (7B)}~\cite{Qwen2-VL}
% & 0.3760 & 0.3625 & 0.3061 & 0.5899
% &-\\
% % $\clubsuit$\textbf{ MiniCPM-V2.6} \cite{}
% % & 0.3733 & 0.1053 & 0.2839 & 0.5916 & 0.5971 & 0.4597
% % &-\\


% $\bigstar$ \textbf{DeepSeekVL (7B)}~\cite{wu2024deepseekvl2mixtureofexpertsvisionlanguagemodels}
% & 0.2611 & 0.3010 & 0.1988
% & 0.2356 
 
% &-\\
    \bottomrule[1pt]
  \end{tabular}}
  \label{mos}
  \vspace{-2em}
\end{table*}

==> tables/real3.tex <==
\begin{table*}
\setlength{\belowcaptionskip}{-0.01cm}
\centering
\belowrulesep=0pt
\aboverulesep=0pt
\renewcommand\arraystretch{1.1}
% \vspace{-6mm}
\caption{{\bf Performance benchmark on AIGVE-60K.} {\it Overall-Averaged} indicates that we average the MOS of the two dimensions as the overall video quality score. $\spadesuit$Conventional handcrafted metrics, $\diamondsuit$VBench metrics, $\clubsuit$deep learning-based VQA models, $\heartsuit$vision-language pre-training models, $\bigstar$open-source LMM-based models, and $\triangle$close-source LMM-based models. $\blacklozenge$*Refers to fine-tuned models. The best results are marked in {\red{RED}} and the second-best in {\blue{BLUE}}. 
% All experiments for AQA and VQA methods are retrained on each dimension under 10 random train-test splits at a ratio of 8:2.
}\vspace{-3mm}
   \resizebox{\linewidth}{!}{\begin{tabular}{l|cc|cc|cc|cc|cc|cc|cc|cc}
    \toprule[1pt]
     %\multicolumn{2}{c}{\bf Training/Testing}&\multicolumn{8}{c}{{\bf GAIA} (9180)}&-\\
     %\midrule
   {\bf Dimension}  & \multicolumn{2}{c|}{\textbf{LIVE}}&\multicolumn{2}{c|}{\textbf{CSIQ}}&\multicolumn{2}{c|}{ \textbf{TID2023}}&\multicolumn{2}{c}{\textbf{KADID}}&\multicolumn{2}{c}{\textbf{CLIVE}}&\multicolumn{2}{c}{\textbf{Koniq}}&\multicolumn{2}{c}{\textbf{Flick8k}}&\multicolumn{2}{c}{\textbf{Overall}}\\
   \cdashline{2-15}
   % \textit{mix with} & \multicolumn{2}{c:}{\textit{Fully AI}} & \multicolumn{2}{c|}{\textit{Partial AI}}& \multicolumn{2}{c:}{\textit{Fully AI}} & \multicolumn{2}{c|}{\textit{Partial AI}}& \multicolumn{2}{c:}{\textit{Fully AI}} & \multicolumn{2}{c|}{\textit{Partial AI}}&\multicolumn{2}{c:}{\textit{Fully AI}} & \multicolumn{2}{c}{\textit{Partial AI}}&\multicolumn{2}{c:}{\textit{Fully AI}} & \multicolumn{2}{c}{\textit{Partial AI}}\\
   % \cdashline{2-15}
{\bf Methods / Metrics}&Acc$\uparrow$&F1$\uparrow$&Acc$\uparrow$&F1$\uparrow$&Acc$\uparrow$&F1$\uparrow$&Acc$\uparrow$&F1$\uparrow$&Acc$\uparrow$&F1$\uparrow$&Acc$\uparrow$&F1$\uparrow$&Acc$\uparrow$&F1$\uparrow$\\
    \midrule
   %  $\spadesuit$BMPRI \cite{quality:BMPRI} &0.5741&0.4976&0.7878&0.7312& 0.3618 &0.3214 &0.7321 &0.6582&0.5106 &0.4452 &0.7709&0.7112 &64.00 &0.7023\\
   %  $\spadesuit$BPRI  \cite{min2017blind}&0.3558 &0.3403 &0.6356 &0.7122 &0.2018& 0.2012 &0.5324 & 0.6256&0.3044&0.2945&0.5800&0.6863&63.56&0.4701\\
   %  $\spadesuit$BRISQUE \cite{mittal2012no} &0.5843&0.4881&0.8131 &0.7196 &0.3806 &0.3325 & 0.7615 & 0.6598&0.5239&0.4459&0.8011&0.7048&64.67&0.7366\\
   % $\spadesuit$HOSA \cite{xu2016blind} &0.6474&0.5642&0.8456&0.7397 &0.4153 & 0.3682 & 0.7780 & 0.6735&0.5773&0.5068&0.8269&0.7226&64.34&0.7571\\
   % $\spadesuit$NIQE \cite{mittal2012making}&0.6536&0.3517&0.8412&0.7500& 0.4345 &0.2544 & 0.7838 & 0.7037 &0.5917&0.3294&0.8251&0.7412&62.21&0.7602\\
   % $\spadesuit$QAC \cite{xue2013learning}&0.5958&0.5717&0.8100&0.7447& 0.3948 & 0.3430 & 0.7717 & 0.6557&0.5421&0.4974&0.8029&0.7182&64.40&0.7495\\
   %  \hdashline
   %  $\diamondsuit$V-Aesthetic Quality~\cite{huang2024vbench}&0.5031 &0.5315 &0.7740 &0.8309 &0.4033 &0.4358 &0.7273 &0.7986 &0.4877 &0.5254 &0.7526& 0.8291&64.54&0.7046\\
   %   $\diamondsuit$V-Imaging Quality~\cite{huang2024vbench}&0.2810 &0.3093 &0.5426 &0.4766 &0.1952 &0.2244 &0.4986 &0.5101 &0.2531 &0.2900 &0.5186 &0.4970&60.60&0.4389\\
   %  $\diamondsuit$V-Overall Consistency~\cite{huang2024vbench}&0.1559 &0.1939 &0.1742 &0.3319 & 0.3076 &0.3685 &0.3201 &0.5419 &0.2510 &0.3046 &0.2338 &0.4233 &61.96&0.3353\\
   %  $\diamondsuit$V-Subject Consistency~\cite{huang2024vbench}& 0.3443 & 0.3968 &0.4839 &0.6065 &0.1647 &0.2425 &0.4416 &0.5744 &0.2739 &0.3476 &0.4679 &0.6016&62.52&0.4545\\
   %   % $\diamondsuit$V-Background Consistency~\cite{huang2024vbench}& 0.3443 & 0.3864 &0.4772 &0.6219 &0.1916 &0.2375 &0.4429 &0.5635 &0.2906 &0.3392 &0.4590 &0.6064&62.37\\
   % $\diamondsuit$V-Temporal Flickering~\cite{huang2024vbench}& 0.4076 &0.4491 &0.6396 &0.6437 &0.1958 &0.2432 &0.5778 &0.5339 &0.3272 &0.3765 &0.6018 &0.6072&63.69&0.5764\\
   %  % $\diamondsuit$Temporal Style~\cite{huang2024vbench}& 0.1559 &0.1939 &0.1742 &0.3319 &0.3076 &0.3685 &0.3201 &0.5419 &0.2510 &0.3046 &0.2338 &0.4233&-\\
   % %  $\clubsuit$Action-Score \cite{liu2023evalcrafter}&&0.2023&0.1823&0.2867&0.2623&0.2689&0.2432&0.2600&0.2377 &-\\
   % % $\clubsuit$Flow-Score \cite{liu2023evalcrafter}& &0.1471&0.1541&0.0816&0.1273&0.1041&0.1309&0.1166&0.1430&-\\
   %     \hdashline
   %  % $\clubsuit$TLVQM \cite{korhonen2019two}&&-\\
   %  % $\clubsuit$VIDEVAL \cite{tu2021ugc}&&-\\
   %  $\clubsuit$VSFA \cite{VSFA}&0.3750 &0.3898 & 0.6227 & 0.5987 &0.2438 &0.2645 &0.5858 &0.5777 &0.3320 &0.3556 &0.6102 &0.5983&57.09&0.5204\\
   %  $\clubsuit$BVQA \cite{li2022blindly}&0.3089 & 0.3512 &0.5030 &0.6506 & 0.2379 & 0.2675 &0.4674 &0.6009 &0.3023 &0.3361 &0.4897 &0.6390&58.47&0.4781\\
   %  $\clubsuit$SimpleVQA \cite{sun2022deep}&0.5631 & 0.5670 & 0.8038 & 0.7873 &0.3474 &0.3487 &0.7273 &0.7327 &0.4884 &0.4979 &0.7620 &0.7756&60.78&0.6894\\
   %  $\clubsuit$FAST-VQA \cite{wu2022fast}&0.6391 & 0.6394 & 0.8945 & 0.9063 & 0.3919 &0.4162 &0.8376 &0.8492 &0.5563 & 0.5738 &0.8683 &0.8952&66.27&0.8122\\ 
   %  $\clubsuit$DOVER \cite{wu2023dover}& 0.6414 & 0.6552 & 0.8874 & 0.9244 &0.3759 &0.3936 &0.8038 &0
   %  .8448 & 0.5480 &0.5702 &0.8496 &0.9043&62.61&0.7662\\
   %   \hdashline
   %   $\heartsuit$CLIPScore~\cite{hessel2021clipscore} &0.0947 &0.1348 &0.0300 &0.1732 &0.2290 & 0.2818 & 0.1408 & 0.3835 &0.1738 &0.2256 &0.0848 &0.2625&58.27&0.1695\\
   %   $\heartsuit$BLIPScore~\cite{li2022blip}&0.1884 &0.2341 &0.2111 &0.3436 &0.3163 &0.3813 & 0.3451 & 0.5354&0.2735 &0.3335 &0.2814 &0.4277&63.93&0.3775\\
   %   $\heartsuit$AestheticScore~\cite{schuhmann2022laion}&0.5524&0.5613 &0.7566 &0.8053 &0.3931 & 0.4149 & 0.7001 & 0.7634 &0.5107 &0.5304 &0.7206 &0.7991&64.87&0.6734\\
   %   % $\heartsuit${\it - - same as the above - -} &&0.3179&0.3101&0.3551&0.3511&0.3504&0.3380&0.3531&0.3458 &-\\
   %   $\heartsuit$ImageReward~\cite{xu2023imagereward}&0.4180 &0.4472 &0.8016 &0.8097 &0.5076 & 0.5419 & 0.8549 & 0.8790&0.4992&0.5365&0.8331&0.8495&68.33&0.8586\\
   %   $\heartsuit$PickScore~\cite{kirstain2023pick}&0.4026 &0.4193 &0.8198 &0.8344 &0.4135 & 0.4246 & 0.7775 & 0.8497&0.4395&0.4580&0.8033&0.8522&62.29&0.7844\\
   %  $\heartsuit$HPSv2~\cite{wu2023human}&0.5415 &0.5690&0.7504&0.8096& 0.4989 & 0.5325 & 0.7522 & 0.8379&0.5605&0.5980&0.7468&0.8325&67.68&0.7789\\
   %  $\heartsuit$VQAScore~\cite{li2024evaluating}&0.1677&0.1961&0.3437&0.3365& 0.1763 & 0.2049 & 0.3922 & 0.4173&0.1880&0.2176&0.3811&0.3746&52.97&0.3280\\
   %  $\heartsuit$FGA-BLIP2~\cite{han2024evalmuse40kreliablefinegrainedbenchmark}&0.5181&0.5340&0.8954&0.8962& 0.5962 & 0.6081 & 0.9502 & 0.9543 &0.6035&0.6196&0.9297&0.9326&67.06&0.9372\\
   %  \hdashline
   %  $\bigstar$DeepseekVL2 (1B)~\cite{wu2024deepseekvl2mixtureofexpertsvisionlanguagemodels}& 0.0121 & 0.0064 & 0.0607 & 0.0427 & 0.0173 & 0.0252& 0.0785 &0.0288&0.0012&0.0137&0.0389&0.0554 & 39.29&0.0965\\
    $\bigstar$DeepseekVL2 (1B)~\cite{wu2024deepseekvl2mixtureofexpertsvisionlanguagemodels}\\
    $\bigstar$LLaVA-1.5 (7B)~\cite{liu2024improved} \\
    $\bigstar$mPLUG-Owl3 (7B)~\cite{ye2024mplug} \\ 
   $\bigstar$MiniCPM-V2.6 (8B)~\cite{yao2024minicpm} \\
   $\bigstar$Qwen2-VL (7B) \cite{wang2024qwen2}\\
 $\bigstar$Qwen2.5-VL (7B)~\cite{Qwen2.5-VL}\\
   $\bigstar$Llama3.2-Vision (11B)~\cite{meta2024llama}\\
  $\bigstar$CogAgent (18B)~\cite{hong2024cogagentvisuallanguagemodel}\\
    $\bigstar$InternVL2.5 (8B)~\cite{chen2024expanding}\\
    $\bigstar$InternVL3 (9B)~\cite{wang2024mpo}\\
   $\bigstar$InternLM-XComposer (7B)~\cite{internlmxcomposer}\\
   $\bigstar$LLaVA-NeXT (8B)~\cite{liu2024llavanext}\\
   $\bigstar$InternVL2.5 (38B)~\cite{chen2024expanding}\\
   $\bigstar$InternVL3 (38B)~\cite{wang2024mpo}\\
   $\bigstar$Qwen2-VL (72B) \cite{wang2024qwen2}\\
   $\bigstar$Qwen2.5-VL (72B)~\cite{Qwen2.5-VL}\\
   $\bigstar$Llava-one-vision (72B)~\cite{xiong2024llavaovchat}\\
   $\bigstar$InternVL2.5 (72B)~\cite{chen2024expanding}\\
   $\bigstar$InternVL3 (72B)~\cite{wang2024mpo}\\
    \hdashline
     $\triangle$Gemini1.5-pro \cite{Gemini}\\
     
     $\triangle$Grok2 Vision \cite{Grok2}\\
% $\bigstar$\textbf{LLaVA-1.5 (7B)}~\cite{wang2025internvideo}
% & 0.3372 & 0.3525 & 0.2577 & 0.3887 
% &-\\
% $\bigstar$\textbf{LLaVA-NeXT (8B)}~\cite{liu2024llavanext}
% & 0.4333 & 0.4164 & 0.3442 & 0.4568 

% &-\\
% $\bigstar$\textbf{mPLUG-Owl3 (7B)}~\cite{ye2024mplug}
% & 0.3918 & 0.3569 & 0.3018 & 0.4744 
% &-\\
% $\bigstar$\textbf{MiniCPM-V2.6 (8B)}~\cite{damonlpsg2025videollama3}
% & 0.3733 & 0.1053 & 0.2839 & 0.5916 
% &-\\
% $\bigstar$\textbf{Qwen2-VL (7B)}~\cite{Qwen2-VL}
% & 0.3760 & 0.3625 & 0.3061 & 0.5899
% &-\\
% % $\clubsuit$\textbf{ MiniCPM-V2.6} \cite{}
% % & 0.3733 & 0.1053 & 0.2839 & 0.5916 & 0.5971 & 0.4597
% % &-\\


% $\bigstar$ \textbf{DeepSeekVL (7B)}~\cite{wu2024deepseekvl2mixtureofexpertsvisionlanguagemodels}
% & 0.2611 & 0.3010 & 0.1988
% & 0.2356 
 
% &-\\
    \bottomrule[1pt]
  \end{tabular}}
  \label{mos}
  % \vspace{-2em}
\end{table*}

==> tables/saliency_ablation.tex <==
\begin{table}[t]
\vspace{-2mm}
  \caption{Ablation study of the proposed LMME3DHF on distortion-aware saliency prediction performance.}
  \label{saliency_ablation}
  \centering
  \vspace{-3mm}
  \resizebox{0.47\textwidth}{!}{
  \begin{tabular}{cl|ccccc}
    \toprule
    No. & Training Strategy & AUC↑ & NSS↑ & CC↑ & SIM↑ & KLD↓
    \\
    \midrule
    (1) & w/o LLM & 0.6233 & 1.1929 & 0.0896 & 0.0716 & 6.3781
    \\
    (2) & Empty Prompt & 0.4574 & 0.0026 & 0.0025 & 0.0127 & 5.0163
    \\
    (3) & Only multimodal features & 0.6587 & 1.1822 & 0.0623 & 0.0203 & 4.4599
    \\
    \rowcolor{gray!20} (4) & \textbf{LMME3DHF (Ours)} & 0.8388 & 6.7689 & 0.5928 & 0.4490 & 1.8759
    \\
    \bottomrule
  \end{tabular}}
\vspace{-2mm}
\end{table}

==> tables/saliency_benchmark.tex <==
\begin{table}[t]
\vspace{-3mm}
  \caption{Performance comparisons of the state-of-the-art saliency models on distortion-aware saliency prediction. The best results are marked in \textcolor{red}{RED} and the second-best in \textcolor{blue}{BLUE}.}
  \label{saliency_benchmark}
  \centering
  \vspace{-3mm}
  \resizebox{0.47\textwidth}{!}{
  \begin{tabular}{l|ccccc}
    \toprule
    Model / Metric & AUC↑ & NSS↑ & CC↑ & SIM↑ & KLD↓
    \\
    \midrule
    \textbf{AIM} \cite{bruce2005saliency} & 0.6374 & 0.7306 & 0.0423 & 0.0163 & 4.6026
    \\
    \textbf{CA} \cite{goferman2011context} & 0.5893 & 0.5113 & 0.0297 & 0.0156 & 4.7227
    \\
    \textbf{CovSal} \cite{erdem2013visual} & 0.5306 & 0.0833 & 0.0051 & 0.0121 & 5.7113
    \\
    \textbf{GBVS} \cite{harel2006graph} & 0.5796 & 0.4507 & 0.0265 & 0.0154 & 4.7863
    \\
    \textbf{HFT} \cite{li2012visual} & 0.5728 & 0.3858 & 0.0223 & 0.0151 & 4.7867
    \\
    \textbf{IT} \cite{itti2002model} & 0.4969 & 0.0822 & 0.0049 & 0.0120 & 7.2030
    \\
    \textbf{Judd} \cite{judd2009learning} & 0.5058 & 0.1850 & 0.0097 & 0.0126 & 4.8111
    \\
    \textbf{Murray} \cite{murray2011saliency} & 0.6251 & 0.6491 & 0.0340 & 0.0146 & 4.6779
    \\
    \textbf{PFT} \cite{guo2008spatio} & 0.5624 & 0.3682 & 0.0185 & 0.0142 & 4.8277
    \\
    \textbf{SMVJ} \cite{cerf2007predicting} & 0.5785 & 0.4426 & 0.0261 & 0.0154 & 4.7884
    \\
    \textbf{SR} \cite{hou2007saliency} & 0.5253 & 0.2517 & 0.0144 & 0.0132 & 4.8328
    \\
    \textbf{SUN} \cite{zhang2008sun} & 0.6291 & 0.7432 & 0.0369 & 0.0156 & 4.6312
    \\
    \textbf{SWD} \cite{duan2011visual} & 0.4907 & 0.1450 & 0.0074 & 0.0125 & 4.9388
    \\
    \midrule
    \textbf{SALICON} \cite{huang2015salicon} & 0.6674 & 0.8193 & 0.0461 & 0.0171 & 4.5764
    \\
    \textbf{Sal-CFS-GAN} \cite{che2019gaze} & \bf\textcolor{blue}{0.7468} & \bf\textcolor{blue}{1.8207}
    & \bf\textcolor{blue}{0.1067} & \bf\textcolor{blue}{0.0441} & \bf\textcolor{blue}{4.1531}
    \\
    \textbf{TranSalNet-ResNet} \cite{lou2022transalnet} & 0.6655 & 0.9245 & 0.0520 & 0.0194 & 4.5461
    \\
    \textbf{TranSalNet-Dense} \cite{lou2022transalnet} & 0.6506 & 1.0633 & 0.0594 & 0.0213 & 4.5431
    \\
    \bottomrule
    \rowcolor{gray!20} \textbf{LMME3DHF (Ours)} & \bf\textcolor{red}{0.8388} & \bf\textcolor{red}{6.7689} 
    & \bf\textcolor{red}{0.5928} & \bf\textcolor{red}{0.4490} & \bf\textcolor{red}{1.8759}
    \\
    \bottomrule
  \end{tabular}}
% \vspace{-5mm}
\end{table}
